Counterfactual Explanations via Latent Space Projection and Interpolation

Counterfactual explanations represent the minimal change to a data sample that alters its predicted classification, typically from an unfavorable initial class to a desired target class. Counterfactuals help answer questions such as "what needs to change for this application to get accepted for a loan?". A number of recently proposed approaches to counterfactual generation give varying definitions of "plausible" counterfactuals and methods to generate them. However, many of these methods are computationally intensive and provide unconvincing explanations. Here we introduce SharpShooter, a method for binary classification that starts by creating a projected version of the input that classifies as the target class. Counterfactual candidates are then generated in latent space on the interpolation line between the input and its projection. We then demonstrate that our framework translates core characteristics of a sample to its counterfactual through the use of learned representations. Furthermore, we show that SharpShooter is competitive across common quality metrics on tabular and image datasets while being orders of magnitude faster than two comparable methods and excels at measures of realism, making it well-suited for high velocity machine learning applications which require timely explanations.

==> 5_checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~General Instructions}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See the Methods section for discussion of latent space on the UCI dataset, and the relatively poor performance on }
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
    \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{Not yet, we require internal review before releasing it.  We have the review process underway now, and will be prepared to add a URL to the camera ready version if the paper is accepted.  Our apologies.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{They are in the appendix.}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{The datasets chosen for this work can be easily computed on commodity hardware.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{All datasets have citations.}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{Release of the code is pending review before open sourcing any repository.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> 7_TODO.tex <==
\section{Things to do}
\subsection{SNIFF TEST}
Things that need to be double checked for fishyness
\begin{itemize}
    \item consistency among CS (classifier shift) in MNIST, UCI, LC
\end{itemize}


\subsection{Models}
\begin{itemize}
    \item LC uae categorical is predicted to be ~0.38 for all samples (M)
    \item Finalize LC - search over klw and categorical loss wt (M)
    \item \sout{Xray TVAE - increase bottleneck capacity (B)}
\end{itemize}


\subsection{Metrics}
\begin{itemize}
    \item Scripts for metrics: IM1 or IM2 (whichever does not involve training a VAE on the base class)
    \item degree of difficulty - try it in input space (not latent) https://arxiv.org/pdf/1910.09398.pdf  - two measure sum over all features, and max difference over all features
    \item connectedness
    \item \sout{closeness - reconstruction loss} - this is what we call proximity
    \item\sout{$x_{cf}-> AE -> recon_loss(x_{cf}, \hat{x}_{cf})$} - this is what we call proximity
    \item \sout{$x_{cf}-> AE -> classification_loss(f(x_{cf})- f( \hat{x}_{cf}))$ }
\end{itemize}

\subsection{Methods}
Investigate external methods we can use as comparisons
\begin{itemize}
    \item Joshi et al REVISE (M)
    \item C-CHVAE (M)
    \item DICE (B) - not sure this works for images ... unless flattened?
    \item AIX360 contrastive (B)
    \item Prototypes/seldon.ai (B)
\end{itemize}

\subsection{UCI fixes}
\begin{itemize}
    \item Change data from binary one-hot-encoding to single dummy ONLY and remove flags
    \begin{itemize}
        \item after data prep file  drop those cols in the make dummies function
        \item Adjust any downstream explicit references to var indices
        \begin{itemize}
            \item Loss functions
            \item some plots
            \item VAE init file output layers
        \end{itemize}
    \end{itemize}
    \item might need more training steps (e.g. $>1200$)
\end{itemize}



\subsection{Writing}
\begin{itemize}
    \item \sout{ABSTRACT  }
    \item update Previous work to include 5 papers mentioned in AIES reviews (B)
    \item Previous work - VAE and generative models
    \item Previous work - mention adversarial (noise, fool classifier) vs CF (substantive change, not trying to trick it)
    
\end{itemize}

\subsection{Figures \& Examples}
\begin{itemize}
    \item would it be useful to have a figure showing interpolation from base to projection, showing alpha and classifier prediction?
    \item MNIST samples - include the label on the left hand side (e.g. original, SS, LGD, FGD, also might be helpful to remind the reader that the counterfactual SHOULD look like the ones generated by SS
    \item tabular examples - save scalers from preproc, histograms of continuous
    \item CF path examples, remove if in need of space?
    
    \item UCI cat fig: normalize to a percentage of total successes.
    \item \sout{map one-hot back to categorical}
    \item \sout{MNIST CF comp: reduce vert white space}
    \item \sout{MNIST CF comparison:  put SS as the row just below the original and have the others below it}

\end{itemize}

\subsection{Appendix Figures}
\begin{itemize}
    \item Diversity of counterfactuals via sampling
    \item Autoencoder comparisons
    \item MNIST and UCI histograms of changes across the methods?
    \item UCI and LC probabilities for a candidate showing non-monotonicity
\end{itemize}


\subsection{Other experiments - discourse - etc.}
\begin{itemize}
    \item What makes the TVAE so useful?  Comparison to nearest target samples, mean of target samples, etc. Also how does the TVAE make its projections (where do the projs end up)? How can we tap into insights from Rep Learning and learning specific representations?
    
    \item wondering how growing spheres handles categoricals...
    \item wondering how GD handles categoricals - especially in latent space.  You'll exploit the continuous variables until what? ...you indavertently trigger a categorical change, then ratchet back the continuous?
    
    \item Closest in latent space metric vs other 9s: why or why not make sense?
\end{itemize}

==> 8_v2TODO.tex <==
\section{Things to do before ArXiv Submission}

\subsection{Overall}

\begin{itemize}
    \item More aggressively make clear a few points that tripped up reviewers
    \begin{itemize}
        \item Why not multi? Why Binary? (place in abstract + intro)
        \item MNIST for inutition, not our focus
        \item One-liner on "this is not causality"
    \end{itemize}
\end{itemize}

\subsection{Abstract}
\begin{itemize}
    \item \sout{Unambiguize lines 1-3}
\end{itemize}

\subsection{Methods}
\begin{itemize}
    \item Add line 147-148 notation to figure 1 and improve labels
    \item \sout{150-153 language too casual}
    \item 161-164: \sout{discuss shortcomings here or later and refer to them} %belongs elsewhere
    \begin{itemize}
        \item \sout{164: tie into the latent dim figures} %belongs elsewhere
    \end{itemize}
    
    \item \sout{End of 164: refer back to experiments and how they reflect} 
    \item \sout{Move in algorithm and refer to it more directly}
    \begin{itemize}
        \item \sout{explain notation for VAEs etc, somehow this got lost}
    \end{itemize}
    \item \sout{Improve captions for Figures 1 + 2}
    
    \item \sout{Add description of comparisons here or in appendix}
    \item \sout{talk about Figures 3 and importance}
    \begin{itemize}
        \item \sout{Move up A.1}
        \item \sout{further explain latent visualizations in "additional views..."}
        \item \sout{Move figure 2 down, expand on figure 3}
        \item \sout{tie in fig 3 to new appendix section}
    \end{itemize}
    \item \sout{refer and explain Figure 2}
    
    \item \sout{One-liner on model training overhead question for time computation}
    \begin{itemize}
        \item \sout{Talk about trade off of model training time vs sample generation time} 
    \end{itemize}
    
    \item \sout{126: explain "adversarial in nature"}

    
\end{itemize}

\subsection{Results}
\begin{itemize}
    \item \sout{191-192: more explanation, maybe relate to multiclass counterfactuals}
    \item \sout{Explain GDI and GDL to a greater extent!}
    \item \sout{Bold the “bests” in the table columns}
    \item \sout{Decrease number of UCI figures}
    \begin{itemize}
        \item \sout{Figure 6 as simple stats or in appendix with references}
        \item \sout{refer to line 232-233 for how to do this}
    \end{itemize}
    
    \item \sout{235: expand LC explanation, background, and takeaways}
    \item \sout{address more directly limitations of our method}
    \begin{itemize}
        \item \sout{In terms of general limitations from conclusion}
        \item \sout{Specific shortcomings results demonstrate}
    \end{itemize}
    
    \item \sout{remove difficulty metric from tables and explanation}
\end{itemize}

\subsection{Conclusion}
\begin{itemize}
    \item \sout{New words for 245-246}
    \item \sout{more about our results and insights}
    \item \sout{remove future work and limitations to a new discussion} section?
\end{itemize}

\subsection{Appendix}
\begin{itemize}
    \item \sout{Add description of comparison methods!}
    \item \sout{Visualizations of SharpShooter Latent Spaces description}
\end{itemize}


\subsection{Minor Final Fixes}
\begin{itemize}
    \item \sout{remove line numbers}
    \item \sout{Add authors + Affil}
    \item \sout{Remove "submitted to" on first page}
    \item \sout{Reorder refs (change style)}
    \item \sout{remove checklist}
    \item \sout{146: missing "that"}
    
\end{itemize}


\section{One-afternoon Fixes}
\begin{itemize}
    \item Fix units on Experiments figures
    \item sparsity fix for MNIST (refer to line 50 in exps/sparsity.py)
    \item Recon loss not reported for UCI
    \item check why sparsity is 0 for UCI-GDI
    
\end{itemize}

\section{Longer-term Improvements}
\begin{itemize}
    %\item Expand upon metrics
    \item Add UCI back to figure 3
    \item consider adding/modifying MNIST figures (potentially more digits)
    \item see 7\_TODO for a more comprehensive list 
\end{itemize}
